An Uncertainty Principle is a Price of Privacy-Preserving Microdata

Privacy-protected microdata are often the desired output of a differentially private algorithm since microdata is familiar and convenient for downstream users. However, there is a statistical price for this kind of convenience. We show that an uncertainty principle governs the trade-off between accuracy for a population of interest ("sum query") vs. accuracy for its component sub-populations ("point queries"). Compared to differentially private query answering systems that are not required to produce microdata, accuracy can degrade by a logarithmic factor. For example, in the case of pure differential privacy, without the microdata requirement, one can provide noisy answers to the sum query and all point queries while guaranteeing that each answer has squared error $O(1/\epsilon^2)$. With the microdata requirement, one must choose between allowing an additional $\log^2(d)$ factor ($d$ is the number of point queries) for some point queries or allowing an extra $O(d^2)$ factor for the sum query. We present lower bounds for pure, approximate, and concentrated differential privacy. We propose mitigation strategies and create a collection of benchmark datasets that can be used for public study of this problem.

==> pratendlowerbound.tex <==

\prAtEndRestateii*
\label{proofsection:prAtEndii}\begin{proof}[]\phantomsection\label{proof:prAtEndii}The lower bounds for pure and approximate DP (but not zCDP) can be proved as consequences of the work of Balcer and Vadhan \cite {Balcer_Vadhan_2019}. To make this material more self-contained, we write out a direct proof of the lower bounds by borrowing their proof technique. \par For notational convenience, we will let $\vec {x}[i]$ denote $q_i(\data )$ (so $\sum _i \vec {x}[i] = \sum _i q_i(\data )=q_*(\data )$). Similarly, we let $\widetilde {\vec {x}}[i]$ denote $q_i(\widetilde {\data })$ (so $\sum _i \widetilde {\vec {x}}[i] = \sum _i q_i(\widetilde {\data })=q_*(\widetilde {\data })$). Thus the vector $\vec {x}$ represents the true point query answers and $\widetilde {\vec {x}}$ represents the privacy protected point query answers. In particular, $\vec {x}$ is a vector of nonnegative integers and $\widetilde {\vec {x}}$ is a vector of nonnegative real numbers. \par All probabilities are taken with respect to only the randomness in $M$. \par In this proof, \underline {$\alpha $, $\beta $, and $k$} are constants that we will set later. For any fixed $j$, by Markov's inequality, \begin {align} P(|\widetilde {\vec {x}}[j] - \vec {x}[j]| \geq \alpha C) \leq \frac {E\left [(\vec {x}[j] - \widetilde {\vec {x}}[j])^2 \right ]}{C^2\alpha ^2}&\leq \frac {1}{\alpha ^2}\label {eq:markovC}\\ P\left (\Big |\sum _{i=1}^{d}\widetilde {\vec {x}}[i] - \sum _{i=1}^{d}\vec {x}[i]\Big | \geq \beta D\right ) &\leq \frac {1}{\beta ^2}\label {eq:markovD} \end {align} \par For each positive integer $n$, positive number $k$, and $i=2,\dots , d$, define the set \begin {align*} G_{i,n,k}&=\left \{\widetilde {\vec {x}} ~:~ \substack {\widetilde {\vec {x}}[i] \in [k, k+2\alpha C],\\ \widetilde {\vec {x}}[1]\in [n-2\alpha C -k, n-k], \\\sum _{j=1}^{d}\widetilde {x}[j] \in [n-\beta D, n+\beta D]}\right \} \end {align*} The intuition behind the meaning of $G_{i,n,k}$ is that suppose we had a dataset $\data _i$ with vector $\vec {x}_i$ of point query answers where the $i^\text {th}$ point query satisfied $\vec {x}_i[i]=k+\alpha C$ and $\vec {x}_i[1]=n-k-\alpha C$ (all other entries are 0) then $G_{i,n,k}$ is the set of all possible outputs $M(\data _i)$ where the $1^\text {st}$ and $i^\text {th}$ entries are within $\alpha C$ of their true value and the sum is within $\beta D$ of its true value. \par For any fixed $n$ and $k$, we next examine how many $G_{i,n,k}$ a vector $\widetilde {\vec {x}}$ can belong to (i.e., an overlap condition). A necessary condition for $\widetilde {\vec {x}}$ to belong to some $G_{i,n,k}$ is that $\widetilde {\vec {x}}[i]\geq k$ and $\widetilde {\vec {x}}[1]\geq n-2\alpha C-k$. This means that after assigning the minimal necessary mass to the $1^\text {st}$ element, there is at most $k+ 2\alpha C +\beta D$ mass to assign to the other elements (without exceeding the upper limit of $n+\beta D$ on the sum of all the cells). Since at least $k$ units of this mass must be assigned to the $i^\text {th}$ element in order for $\widetilde {\vec {x}}$ to belong to $G_{i,n,k}$, this means that $\vec {\widetilde {x}}$ can belong to $G_{i,n,k}$ for at most $\frac {2\alpha C+\beta D +k}{k}$ different choices of $i$. \par Now define $ \vec {x}_1,\dots , \vec {x}_{d}$ as follows. $\vec {x}_1[1]=n$ with all other entries being $0$. Next for $i=2,\dots ,d$ we set $\vec {x}_i[1]=n-\alpha C - k$ and $\vec {x}_i[i]=\alpha C + k$ and all other entries of $\vec {x}_i$ are 0. For each $i$, Let $\data _i$ be a database whose point query answers are $\vec {x}_i$, which is possible since the point queries are disjoint (and this means that $\data _1$ differs from all of the others by the addition/removal of at least $2(\alpha C + k)$ records). \par \textbf {For pure differential privacy}, we have: \begin {align*} 1 &\geq P\left (M(\data _1) \in \bigcup _{i=2}^{d}G_{i,n,k}\right ) \geq \frac {k}{2\alpha C + \beta D+k} \sum _{i=2}^{d} P\left (M(\data _1) \in G_{i,n,k}\right ) \text { by overlap condition}\\ &\geq e^{-\epsilon 2(\alpha C+k)} \frac {k}{2\alpha C + \beta D+k}\sum _{i=2}^{d} P\left (M(\data _i) \in G_{i,n,k}\right ) \text { by group privacy property of $\epsilon $-DP \cite {diffpbook}}\\ &\geq e^{-\epsilon 2(\alpha C+k)} \frac {k}{2\alpha C + \beta D+k}\sum _{i=2}^{d} \left (1 - \frac {2}{\alpha ^2}-\frac {1}{\beta ^2}\right ) \text { by the Markov inequality and union bound}\\ &= e^{-\epsilon 2(\alpha C+k)} \frac {k(d-1)}{2\alpha C + \beta D+k} \left (1 - \frac {2}{\alpha ^2}-\frac {1}{\beta ^2}\right ) \end {align*} \par Now we set $\alpha =2$ and $\beta =2$ to get \par \begin {align*} e^{2\epsilon (2C + k)} \geq \frac {k(d-1)}{16C + 8D + 4k} \end {align*} If $D$ is allowed to be $\leq C$, then we set $k=C$ and get \begin {align*} e^{6\epsilon C} &\geq \frac {d-1}{28} &&\Rightarrow & C &\geq \frac {1}{6\epsilon }\log \frac {d-1}{28} \end {align*} In general, if $D\in O(C)$ (i.e., $D$ is allowed to be at most some constant times $C$) then similar arguments show $C\in \Omega \left (\frac {1}{\epsilon }\log (d)\right )$. \par If $D$ is allowed to be $> C$ then we set $k=1/\epsilon $ and get \begin {align*} e^{4\epsilon C + 2} &\geq \frac {(d-1)}{24\epsilon D + 4} &&\Rightarrow &C &\geq \frac {1}{4\epsilon } \left (\log \left (\frac {(d-1)}{24\epsilon D + 4}\right )- 2\right ) \end {align*} In general, if $D\in \Omega (C)$ (i.e., $D$ is required to be at least some constant times $C$) then similar arguments show that $C\in \Omega \left (\frac {1}{\epsilon }\log (\frac {d}{\epsilon D})\right )$. \par Putting these facts together, we see that if $D\in O(1/\epsilon )$ then $C\in \Omega (\frac {1}{\epsilon }\log (d))$. Meanwhile, if $C\in O(1/\epsilon )$ then we must have $D\in \Omega (d/\epsilon )$. \par \par \textbf {For approximate, differential privacy}, using the group privacy property of approximate differential privacy \cite {Balcer_Vadhan_2019}, \begin {align*} 1 &\geq P\left (M(\data _1) \in \bigcup _{i=2}^{d}G_{i,n,k}\right ) \geq \frac {k}{2\alpha C + \beta D+k} \sum _{i=2}^{d} P\left (M(\data _1) \in G_{i,n,k}\right ) \\ &\geq \frac {k}{2\alpha C + \beta D+k}\sum _{i=2}^{d} \left (e^{-\epsilon 2(\alpha C+k)}P\left (M(\data _i) \in G_{i,n,k}\right ) - \delta /\epsilon \right ) \text { by group privacy}\\ &\geq \frac {k}{2\alpha C + \beta D+k}\sum _{i=2}^{d} \left (e^{-\epsilon 2(\alpha C+k)}\left (1-\frac {2}{\alpha ^2}-\frac {1}{\beta ^2}\right ) - \delta /\epsilon \right ) \text { Markov inequality, union bound}\\ &= \frac {k(d-1)}{2\alpha C + \beta D+k} \left (e^{-\epsilon 2(\alpha C+k)}\left (1-\frac {2}{\alpha ^2}-\frac {1}{\beta ^2}\right ) - \delta /\epsilon \right )\\ \end {align*} Setting $\alpha =2$ and $\beta =2$ gives \begin {align*} 1 \geq \frac {k(d-1)}{4 C + 2 D+k} \left (\frac {1}{4}e^{-\epsilon 2(2 C+k)} - \delta /\epsilon \right ) \text { and so } \left (1+\frac {\delta }{\epsilon }\; \frac {k(d-1)}{4 C + 2 D+k} \right )e^{4\epsilon C + 2k\epsilon } &\geq \frac {1}{4}\;\frac {k(d-1)}{4 C + 2 D+k} \end {align*} and this is the same as \begin {align*} \left (\frac {\delta }{\epsilon } + \frac {4C + 2D + k}{k(d-1)}\right )e^{4\epsilon C + 2k\epsilon } \geq 1/4 \end {align*} Noting that for any $z$, $1+z\leq 2\max \left (1, z\right )$ and so \begin {align*} e^{4\epsilon C + 2k\epsilon } &\geq \frac {1}{8}\min \left (\frac {k(d-1)}{4 C + 2 D+k},\; \frac {\epsilon }{\delta }\right )\\ \end {align*} Proceeding as we did for pure differential privacy, if $D$ is allowed to be $O(C)$, then $C\in \Omega \left (\min \left ( \frac {1}{\epsilon }\log (d),\;\frac {1}{\epsilon }\log \frac {\epsilon }{\delta } \right )\right )$; if $D$ is allowed to be $\Omega (C)$ then $C\in \Omega \left (\min (\frac {1}{\epsilon }\log \frac {d}{\epsilon D},\;\frac {1}{\epsilon }\log \frac {\epsilon }{\delta })\right )$. \par Putting this together, if $D\in O(1/\epsilon )$ then $C\in \Omega \left (\min \left ( \frac {1}{\epsilon }\log (d),\;\frac {1}{\epsilon }\log \frac {\epsilon }{\delta } \right )\right )$ and if $C\in O(1/\epsilon )$ then either $\epsilon \in O(\delta )$ or $D\in \Omega (d/\epsilon )$. \par \textbf {For $\rho $-zCDP}, consider a random variable $X$ that is uniform over $\data _2,\dots ,\data _{d}$ (i.e., with probability $1/(d-1)$, $X$ is the dataset $\data _i$). Note that the $\data _i$ we have been using can be constructed so that $i\neq j$, $\data _i$ and $\data _j$ differ on the addition/removal of $2aC + 2k$ people. Let $I(\cdot ; \cdot )$ denote mutual information and $H(\cdot )$ denote entropy. By the group privacy property of zCDP \cite {zcdp} we have two facts relating group privacy to mutual information: (1) $\rho (2\alpha C + 2k)^2 \geq I(M(\vec {\data }_i); M(\vec {\data }_j))$ for all $i$ and $j$ (from Proposition 5.3 proof in \cite {zcdp}) and (2) the corollary that $\rho (2\alpha C + 2k)^2 \geq I(X, M(X))$ (from Proposition 6.1 proof in \cite {zcdp}). Then \par \begin {align} \rho (2\alpha C + 2k)^2 &\geq I(X; M(X)) = H(X) - H(X ~|~M(X))\nonumber \\ &= \log _2(d-1)- H(X ~|~M(X))\label {eq:zcdp_part1} \end {align} and now we need to upper bound $H(X~|~M(X))$. Define $G$ to be the event that $M(X)$ is in the $G_{i,n,k}$ that corresponds to the realized value of $X$ (i.e., the event $X=\data _j \Rightarrow M(X)\in G_{j,n,k}$ for $j=2,\dots , d$). Then we obtain a Fano-like inequality (following the proof structure in \cite {cover}) as follows: \begin {align} H(X~|~M(X))&= H(X~|~M(X)) + H(G~|~X, M(X))\nonumber \\ &\quad \text {(the last entropy is 0 since $G$ is a deterministic function of $X$ and $M(X)$)}\nonumber \\ &= H(G, X ~|~M(X)) \quad \text { by the chain rule for conditional entropy}\nonumber \\ &= H(G~|~M(X)) + H(X ~|~ G, M(X))\quad \text { by chain rule for conditional entropy}\nonumber \\ &\leq 1 + H(X ~|~ G, M(X)) \quad \text { since G is binary, its entropy is $\leq 1$}\nonumber \\ &=1 + P(G=0)H(X~|~M(X), G=0) + P(G=1)H(X~|~M(X), G=1)\nonumber \\ &\leq 1 + P(G=0)\log _2(d-1)+ P(G=1)H(X~|~M(X), G=1)\nonumber \\ &\quad \text {(since the entropy of $X$ is $\leq \log _2(d-1)$ )}\nonumber \\ &\leq 1 + P(G=0)\log _2(d-1)+ P(G=1)\log _2\left (\frac {2\alpha C + \beta D + k}{k}\right )\nonumber \\ &\text {(This follows from $G=1$, by the overlap condition, since then $M(X)$ can }\nonumber \\ &\text {belong to at most $\frac {2\alpha C + \beta D + k}{k}$ of the $G_{i,n,k}$ so conditioned on knowing $M(X)$}\nonumber \\ &\text {there are at most $\frac {2\alpha C + \beta D + k}{k}$ possible choices for $X$ }\nonumber \\ &\text {and hence $\log _2$ of this quantity upper bounds the conditional entropy)}\nonumber \\ &\leq 1 + P(G=0)\log _2(d-1) + \log _2\left (\frac {2\alpha C + \beta D + k}{k}\right )\nonumber \\ &\leq 1 + (\frac {2}{\alpha ^2} + \frac {1}{\beta ^2})\log _2(d-1) + \log _2\left (\frac {2\alpha C + \beta D + k}{k}\right )\label {eq:zcdp_part2} \end {align} Where the last inequality follows from the Markov inequality and union bound on $P(G=0)$. Now, setting $\alpha =\beta =2$ and combining Equations \ref {eq:zcdp_part1} and \ref {eq:zcdp_part2}, we have: \par \begin {align*} \rho (4 C + 2k)^2 \geq \frac {1}{4}\log _2(d-1) - \log _2\left (\frac {4 C + 2 D + k}{k}\right ) - 1 \end {align*} \par \par \par \underline {If $D$ is allowed to be $\leq C$\mystrut }, we set $k=C$ to get \par \begin {align*} \rho (6C)^2 &\geq \frac {1}{4}\log _2(d-1) - \log _2\left (\frac {4 C + 2 D + C}{C}\right ) - 1 \geq \frac {1}{4}\log _2(d-1) - \log _2\left (\frac {7C}{C}\right ) - 1\\ &\geq \frac {1}{4}\log _2(d-1)-4 \Rightarrow C\geq \frac {1}{6\sqrt {\rho }}\sqrt {\frac {\log _2(d-1)}{4} - 4} \end {align*} \par so in general, if $D\in O(C)$ then similar arguments show that $C\in \Omega \left (\sqrt {\frac {1}{\rho }\log (d)}\right )$. \par \underline {If $D$ is allowed to be $> C$\mystrut }, then let $\gamma $ be any number strictly between $0$ and $1$. Then we set $k=1/\sqrt {\rho }$, and $\alpha =\beta =\sqrt {\frac {3}{(1-\gamma )}}$. Combining Equations \ref {eq:zcdp_part1} and \ref {eq:zcdp_part2} \begin {align*} \lefteqn { (2\alpha \sqrt {\rho } C + 2)^2}\\ &\geq \left (1-\frac {2}{\alpha ^2} - \frac {1}{\beta ^2}\right )\log _2(d-1) - \log _2\left (2\alpha \sqrt {\rho } C + \beta \sqrt {\rho } D + 1\right ) - 1\\ &=\gamma \log _2(d-1) - \log _2\left (2\alpha \sqrt {\rho } C + \beta \sqrt {\rho } D + 1\right ) - 1\\ &\geq \gamma \log _2(d-1) - \log _2\left (3\sqrt {\frac {3}{1-\gamma }} \sqrt {\rho }D + 1\right ) - 1 \end {align*} which implies \begin {align*} C \geq \sqrt {\frac {1-\gamma }{12}}\sqrt {\frac {\gamma \log _2(d-1) - \log _2(3\sqrt {\frac {3}{1-\gamma }}\sqrt {\rho }D + 1) - 1}{\rho }} - \frac {1}{\sqrt {\rho }}\sqrt {\frac {1-\gamma }{3}} \end {align*} \par \par In general, if $D$ is allowed to be $\Omega (C)$ then similar arguments show that $C\in \Omega \left (\sqrt {1-\gamma }\sqrt {\frac {\gamma \log _2(d-1) - \log _2(\sqrt {\frac {3}{1-\gamma }}\sqrt {\rho }D + 1) - 1}{\rho }} - \frac {1}{\sqrt {\rho }}\sqrt {\frac {1-\gamma }{3}}\right )$. \par Putting all of this together, if $D\in O(1/\sqrt {\rho })$ then $C\in \Omega \left (\sqrt {\log (d)/\rho }\right )$. But in order to get $C=O(1/\sqrt {\rho })$, we must have $D\in \Omega (d^\gamma /\sqrt {\rho })$. \par \end{proof}


==> pratendupperbound.tex <==

\prAtEndRestateiii*
\label{proofsection:prAtEndiii}\begin{proof}[]\phantomsection\label{proof:prAtEndiii}The double-sided geometric mechanism $DGeo(\epsilon )$ is a discrete version of the Laplace distribution, supported over integers, with probability mass function $p(k)= \frac {1-e^{-\epsilon }}{1+e^{-\epsilon }}e^{-\epsilon |k|}$ \cite {GRS09}. It has several useful properties: (a) its mean is 0, (b) its variance is $2\frac {e^{-\epsilon }}{(1-e^{-\epsilon })^2}\leq 2/\epsilon ^2$, (c) given an integer-valued query $q$, adding $DGeo(\epsilon /\Delta _1(q))$ to its answer satisfies $\epsilon $-differential privacy. \par Similarly, the discrete Gaussian $DGauss(0, 1/(2\rho ))$ is a discrete version of the Gaussian distribution \cite {dgm} with several useful properties: (a) its mean is 0, (b) its variance is less than that of $N(0, 1/(2\rho ))$, (c) given an integer-valued query $q$, adding $DGauss(0, \Delta _2(q)^2/(2\rho ))$ to its answer satisfies $\rho $-zcdp. \par \textbf {To prove Item \ref {item:dppoint}}, let $r_1,\dots , r_d$ be records satisfying the predicates for point queries $q_1,\dots , q_d$, respectively. Let $M_\epsilon $ be the algorithm that first computes nonnegative noisy query answers $a_i = \max \{0, q_i(\data ) + DGeo(1/\epsilon )\}$ for $i=1,\dots , d$ and then outputs the synthetic dataset $\widetilde {\data }$ that has $a_i$ copies of record $r_i$ for each $i$. Note that $M_\epsilon $ does not obtain a noisy answer to $q_*$, and so it satisfies $\epsilon $-differential privacy since $\Delta _1(q_1,\dots , q_d)=1$ Since $q_i(\data )\geq 0$ for all $i$, we have: \begin {align*} E\left [(q_i(\data )-q_i(M_\epsilon (\data )))^2\right ] &= E\left [(q_i(\data ) - \max \{0, q_i(\data )+DGeo(\epsilon )\})^2\right ]\\ &\leq E\left [(q_i(\data ) - (q_i(\data )+DGeo(\epsilon )))^2 \right ]\leq 2/\epsilon ^2\\ \end {align*} Furthermore \begin {align*} \lefteqn {E\left [(q_*(\data ) - q_*(M_\epsilon (\data )))^2\right ] = E\left [(\sum _i q_i(\data )-\sum _i q_i(M_\epsilon (\data )))^2\right ]}\\ &= \sum _i E\left [(q_i(\data ) - \max \{0, q_i(\data )+DGeo(\epsilon )\})^2\right ]\\ &\phantom {=} + 2\sum _{i,j: i < j} E\left [\Big (q_i(\data ) - \max \{0, q_i(\data )+DGeo(\epsilon )\}\Big )\right ]E\left [\Big (q_j(\data ) - \max \{0, q_j(\data )+DGeo(\epsilon )\}\Big )\right ]\\ &\leq d \frac {2}{\epsilon ^2} + d(d-1)\frac {2}{\epsilon ^2} = d^2\frac {2}{\epsilon ^2} \end {align*} \par \textbf {To prove Item \ref {item:zcdppoint}}, we use the same proofs as before, except that $M_\rho $ synthesizes $\widetilde {\data }$ using the noisy answers $a_i=q_i(\data ) + \max \{0, DGauss(0, 1/(2\rho ))\}$. Following essentially the same calculations, we see that the expected squared error of each point query $q_i$ is at most $1/(2\rho )$ and for the sum query $q_*$ it is at most $d^2/(2\rho )$. \par \textbf {To prove Item \ref {item:dpsum}}, let $r_1,\dots , r_d$ be records satisfying the predicates for point queries $q_1,\dots , q_d$, respectively. Let $M^\prime _\epsilon $ be the algorithm that does the following. First, it obtains noisy answers for each query: $a_i = q_i(\data ) + Lap(2/\epsilon )$ for $i=1,\dots , d$ and $a_*= q_*(\data ) + Lap(2/\epsilon )$. (Since $\Delta _1(q_1,\dots , q_d, q_*)=2$, this clear satisfies $\epsilon $-differential privacy). Next, $M$ solves the following optimization problem: \par \begin {align*} \arg \min _{x_1,\dots , x_d} &\frac {1}{2}\sum _{i=1}^d (x_i-a_i)^2\\ \text {s.t. } &\sum _{i=1}^d x_i = \max \{0, a_*\}\\ \phantom {\text {s.t. }} &x_i\geq 0, \text { for $i=1,\dots , d$} \end {align*} and creates a privacy protected microdata $\widetilde {\data }$ that consists of the records $r_1,\dots , r_d$ with respective weights $x_1,\dots , x_d$. \par Since the sum query is nonnegative and the problem is constrained so that $\sum _i x_i$ is equal to $\max \{0, a_*\}$, clearly $E\left [(q_*(M^\prime _\epsilon (\data )) - q_*(\data ))^2\right ]\leq 2/\epsilon ^2$. \par Now let us derive an upper bound on $E\left [(q_i(M^\prime _\epsilon (\data )) - q_i(\data ))^2\right ]$ for a point query $q_i$. \par For each $i$, let $z_i=a_i-q_i(\data )$ and $z_*= a_*-q_*(\data )$ be the actual noises that are added (they are all i.i.d. Laplace$(2/\epsilon )$. \par We know from Lemma \ref {lem:cnnls} that the solution $x_i$ have the form $\max \{a_i-\gamma , 0\}$ (which is $\max \{0, q_i(\data )+z_i-\gamma \}$) for some $\gamma $ such that $\sum _i \max \{a_i-\gamma , 0\}=\max \{0, a*\}$ and note that the left hand side is monotonic in $\gamma $. \par We first find a suitable upper and lower bound on $\gamma $. Define $L=-|z_*| + \min _i z_i$ and $U=|z_*|+ \max _i z_i$. Then we have: \begin {align*} \sum _i \max \{0, a_i - U\} &= \sum _i \max \{0, q_i(D)+z_i-U\}\leq \sum _i\max \{0, q_i(\data ) - |z_*|\}\\ &\leq \max \{0, \left (\sum _i q_i(\data )\right ) - |z_*|\}\\ &\text {since the $q_i(\data )$ are nonnegative}\\ &= \max \{0, q_*(\data ) - |z_*|\}\\ &\leq \max \{0, a_*\} \end {align*} and so $\gamma \leq U$. \par Next, \begin {align*} \sum _i \max \{0, a_i - L\} &= \sum _i \max \{0, q_i(D)+z_i-L\}\geq \sum _i\max \{0, q_i(\data ) + |z_*|\}\\ &= \sum _i\left ( q_i(\data ) + |z_*|\right )\\ &\text {since the $q_i(\data )$ are nonnegative}\\ &\geq \left (\sum _i q_i(\data )\right ) + |z_*|\\ &=q_*(\data ) + |z_*|\geq \max \{0, a_*\} \end {align*} and so $\gamma \leq L$. \par \par We next find a bound on $E\left [(q_i(M^\prime _\epsilon (\data )) - q_i(\data ))^2\right ]$ in terms of $\gamma $. \begin {align} E\left [(q_i(M^\prime _\epsilon (\data )) - q_i(\data ))^2\right ] &= E\left [(\max \{0, q_i(\data )+z_i-\gamma \} - q_i(\data ))^2\right ]\nonumber \\ &\text { note the random variable here are $z_i$ and $\gamma $}\nonumber \\ &\leq E\left [(( q_i(\data )+z_i-\gamma ) - q_i(\data ))^2\right ]\nonumber \\ &\text { since $q_i(\data )$ is nonnegative and removing the max moves the}\nonumber \\ &\text { left part further away from $q_i(\data )$}\nonumber \\ &=E\left [(z_i-\gamma )^2 \right ]\leq E\left [\left (|z_i| + \max \{|L|, |U|\}\right )^2\right ]\nonumber \\ &\leq E\left [\left (|z_i| + |z|_* + \max _j |z_j|\right )^2\right ]\nonumber \\ &\text {since the noises $z_j$ are symmetric around 0}\nonumber \\ &\leq E\left [\left (|z|_* + 2\max _j |z_j|\right )^2\right ]\nonumber \\ &=E\left [z_*^2\right ] + 4E\left [|z_*|\right ]E\left [\max _j |z_j|\right ] + 4E\left [(\max _j |z_j|)^2\right ]\label {eq:commonproof}\\ &\in O(\frac {1}{\epsilon ^2}\log ^2(d)) \quad \text {by Lemma \ref {lem:distributions} for Laplace noise}\nonumber \end {align} \par \textbf {To prove Item \ref {item:zcdpsum}} we follow the same steps as before, but using $N(0, 1/(\rho ))$ noise instead of Lap$(2/\epsilon )$ (noting that $\Delta _2(q_1,\dots , q_d, q_*)=\sqrt {2}$) and again see that the variance of the sum query is at most $1/\rho $, while for the point queries, the only thing that changes are the calculations after Equation \ref {eq:commonproof}, where we use the Lemma \ref {lem:distributions} results for Gaussian noise, to conclude that $E[(q_i(\data ) - q_i(M(\data )))^2]\in O(\frac {1}{\rho }\log (d))$ for each $i$. \par \textbf {To prove Item \ref {item:appsum}}, we again follow the same steps as before but with a different noise distribution. Recall that the double geometric distribution $DGeo(\epsilon )$ is supported over the integers. If $z\sim DGeo(\epsilon )$ then $P(z=k) = \frac {1-e^{-\epsilon }}{1+e^{-\epsilon }}e^{-\epsilon |k|}$. Furthermore, if $k\geq 0$, $P(z \geq k) = P(z \leq -k) = \frac {1}{1+e^{-\epsilon }}e^{-\epsilon k}$. \par For any integer $B> 0$, the truncated double geometric distribution $TDGeo(\epsilon , B)$ is obtained by clipping a DGeo$(\epsilon )$ at $B$ and $-B$. Specifically, if $z'\sim TDGeo(\epsilon , B)$ then \begin {align*} P(z^\prime = k) &= \begin {cases} \frac {1}{1+e^{-\epsilon }}e^{-\epsilon B} & \text { if }k=B\\ \frac {1-e^{-\epsilon }}{1+e^{-\epsilon }}e^{-\epsilon |k|} & \text { for $k=-B+1, \dots , B-1$}\\ \frac {1}{1+e^{-\epsilon }}e^{-\epsilon B} & \text { if }k=-B\\ \end {cases} \end {align*} \par So, we follow the same approach as in the proof of Item \ref {item:dpsum} but we use $TDGeo(\epsilon /2, B)$ noise to answer each query (detail queries and sum query). We first determine the value of $B$ needed to satisfy $(\epsilon /2,\delta /2)$-DP. \par First note that for any integer $v$, and integer $k\in [v-B+1, v+B-2]$ $$e^{-\epsilon /2}\leq \frac {P(v+TDGeo(\epsilon /2, B)=k)}{P(v-1+TDGeo(\epsilon /2, B)=k)} \leq e^{\epsilon /2}$$ (the significance of these points are that they are not in the boundary of $v+TDGeo$ or $v-1+TDGeo$). \par \par Meanwhile $P(v+TDGeo(\epsilon /2)\in \{v-B, v+B-1, v+B\}) = P(DGeo(\epsilon /2) \geq B-1) + P(DGeo(\epsilon /2) \leq -B)= \frac {1}{1+e^{-\epsilon /2}}e^{-\epsilon B/2} + \frac {1}{1+e^{-\epsilon /2}}e^{-\epsilon (B-1)/2}\leq 2e^{-\epsilon (B-1)/2}$. These are the boundary points where the probability ratios may be large. \par Setting this equal to $\delta /2$ (and then performing similar calculations when the $v-1$ term is in the numerator), we see that adding $TDGeo(\epsilon /2, B)$ noise satisfies $\epsilon ,\delta $-DP if $B\geq \frac {2}{\epsilon }\log (4/\delta )+1$. \par Thus using a naive composition result of approximate differential privacy \cite {diffpbook}, we can add TGeo$(\epsilon /2, B)$ noise to each point query and the sum query to satisfy $(\epsilon ,\delta )$-DP. \par Using the same postprocessing as in the proof of Item \ref {item:dpsum}, we see that the expected squared error of the sum query (when computed from the postprocessed privacy-protected data) is at most variance$(TDGeo(\epsilon /2, B))\leq $ variance$(DGeo(\epsilon /2))\leq 8/\epsilon ^2$. \par For the point queries, the only thing that changes are the calculations after Equation \ref {eq:commonproof}. Since the absolute value of the noises is bounded by $B$, we get that the expected squared error of the point queries is $\in O(B^2)=O(\frac {1}{\epsilon ^2}\log ^2(1/\delta )+1)$. \par \end{proof}

